Modeling Supply and Demand in Public Transportation Systems

We propose two neural network based and data-driven supply and demand models to analyze the efficiency, identify service gaps, and determine the significant predictors of demand, in the bus system for the Department of Public Transportation (HDPT) in Harrisonburg City, Virginia, which is the home to James Madison University (JMU). The supply and demand models, one temporal and one spatial, take many variables into account, including the demographic data surrounding the bus stops, the metrics that the HDPT reports to the federal government, and the drastic change in population between when JMU is on or off session. These direct and data-driven models to quantify supply and demand and identify service gaps can generalize to other cities' bus systems.

==> Sections/1_introduction/model_overview.tex <==
\subsection{Overview of the Models}

==> Sections/1_introduction/paper_structure.tex <==
\subsection{Structure of the Paper}

==> Sections/2_methods/limitations.tex <==
\subsection{Limitations for the Models}

%The models constructed will naturally have limitations due to the complex nature of the transit system. Among these includes the time constraint of eight weeks for this project to be completed. This led us to prioritize certain outcomes and to be limited on solving certain issues we encountered since we did not have unlimited time to fix problems that occurred, especially those that happened towards the end of the eight-week period. 

%Furthermore, the circumstance of Harrisonburg's population is not applicable to all cities of similar size.  Harrisonburg, VA is a city that has a shifting population; since it is a college town, the population of the city is reliant both on residents and students of the city. Thus, these models take this into account and would be best applied to other areas with similar circumstances. The assumptions on the data also provide limitations to these models. In regards to the fluctuation of Harrisonburg population, it was assumed that 90\% of JMU students that do not have a summer class do not remain in Harrisonburg over the summer break. The 90\% value is strictly an arbitrary approximation; 

this was based on inference and deductive reasoning from us and is not reflected in a methodical study. To improve the accuracy of the population adjustments, it is advised to further investigate the true value of students remaining in the location being studied when the university is not in session. 

In regards to the social vulnerability variables data being initially collected in block groups and then being transformed into blocks, the assumption was made that the variables could be evenly redistributed into the blocks based on their population proportions within their respective block groups. This proves to be a limitation since these assumed values need to be compared with the true data of the social vulnerability variables originally partitioned into blocks to determine if this assumption accurately reflects the condition of the community within the block. Finally, the social vulnerability variables selected from the fifteen factors in the social vulnerability index were chosen based upon our discretion as researchers. They were chosen based upon our intuition of what, logically, would impact transit ridership. With this process, there may be a factor we excluded from this model that may influence ridership and this should be taken into account when using our methodology.


==> Sections/2_methods/we_didnt_use.tex <==
\subsection{Additional Research}
While exploring the trends in the data collected and brainstorming possible variables for our models, we looked into a multitude of factors and data sets to give us perspective on the information we were working with. As we began narrowing down the data we would be using to build our models, certain information that was collected was determined to not be directly included in them. However, the research is still valuable to the project because it was vital to the beginning stages of the models; thus, we have included these in subsections below to provide context and insight into our process.

\subsubsection{Data Obtained by Census Tract}

Census tracts are a spatial unit used by the U.S. Census Bureau when measuring factors like population. Harrisonburg is divided into 11 census tracts. Census tracts are then divided into block groups, of which Harrisonburg has 27. The smallest spatial unit that data is reported in is blocks, which are a subdivision of block groups. Harrisonburg is divided into 631 blocks. Much of the initial data collected was reported by census tract. However, it was determined that data by block would provide a more accurate model of Harrisonburg. Therefore, we decided to exclude data reported by census tract and instead collected new data by smaller spatial units.

\subsubsection{SVI Calculation}
    
The social vulnerability index (SVI) is a measure used by the Center for Disease Control (CDC) and other government institutions to measure potential adverse effects to humans by external pressures. The measure itself is a positive number ranging from 0 to 1, with 0 indicating low social vulnerability and 1 indicating high social vulnerability. According to \cite{atsdr2022CDC},

\begin{quote}
    Every community must prepare for and respond to hazardous events, whether a natural disaster like a tornado or disease outbreak, or a human-made event such as a harmful chemical spill. A number of factors, including poverty, lack of access to transportation, and crowded housing may weaken a community’s ability to prevent human suffering and financial loss in a disaster. These factors are known as social vulnerability.
\end{quote}

The CDC calculates the social vulnerability of a community based on 15 factors, grouped into four themes. These factors are as follows: 

\begin{minipage}[t]{0.45\textwidth}
\begin{itemize}
    \item Socioeconomic Status
    \begin{itemize}
        \item Below Poverty 
        \item Unemployed 
        \item Income 
        \item No High School Diploma 
    \end{itemize}
    
    \item Household Composition \& Disability
    \begin{itemize}
        \item Age 65 or Older 
        \item Age 17 or Younger 
        \item Older Than Age 5 With a Disability 
        \item Single-Parent Households 
    \end{itemize}
\end{itemize}
\end{minipage}
\begin{minipage}[t]{0.45\textwidth}
\begin{itemize}
    \item Minority Status \& Language
    \begin{itemize}
        \item Minority 
        \item Speaks English ``Less Than Well'' 
    \end{itemize}
    
    \item Housing \& Transportation
    \begin{itemize}
        \item Multiunit Structures 
        \item Mobile Homes 
        \item Crowding 
        \item No Vehicle 
        \item Group Quarters
    \end{itemize}
\end{itemize}
\end{minipage}
\vspace{1em}

% The CDC's social vulnerability index can be used to determine whether transit services are meeting the demands and needs of social vulnerable demographics, such as persons older than 65 years or those with disabilities. 

As of 2018, the city of Harrisonburg retains a SVI of 0.79, indicating a medium to high level of social vulnerability. A more detailed description of SVI per census tract is given in Table \ref{tab:census_tract_svi} and this is visually represented in Figure \ref{fig:svi_map}. In general, SVI is a helpful tool to understand the city, but the data is only available by census tract. Meanwhile, we hope to assess transit supply and demand by census block. Instead of using the index itself, we extracted select factors, which we deemed social vulnerability variables (SVV), to include in our models.

\begin{table}[ht]
	\begin{minipage}{0.5\linewidth}
		    \caption{A table of SVI for Harrisonburg, VA by census tract.}
            \label{tab:census_tract_svi}
		\centering
    \begin{tabular}{c c c}
        Census Tract & Population & SVI \\
        \hline
        1.01 & 5015 & 0.7236 \\
        1.02 & 5696 & 0.7282 \\
        2.03 & 1901 & 0.2533 \\
        2.04 & 4430 & 0.7931 \\
        2.05 & 6001 & 0.2650 \\
        2.06 & 4725 & 0.0761 \\
        2.07 & 6231 & 0.7299 \\
        3.01 & 3575 & 0.1122 \\
        3.02 & 5679 & 0.8001 \\
        4.01 & 3577 & 0.8111 \\
        4.02 & 6561 & 0.7432
    \end{tabular}
	\end{minipage}\hfill
	\begin{minipage}{0.45\linewidth}
		\centering
		\captionof{figure}{A map of SVI for Harrisonburg, VA by census tract}
		\label{fig:svi_map}
		\includegraphics[width=75mm]{Images/maps/arcgis_svi.pdf}
	\end{minipage}
\end{table}


\subsubsection{JMU Parking}

Initially, it was thought that the amount of parking spaces available to JMU students would impact ridership of public transportation. This idea was mentioned by the assistant director of the HDPT in a meeting and we decided to investigate how parking decks and parking space availability influenced ridership. Data on the number of available parking spaces on-campus and the daily usage of these parking spaces were originally requested from the JMU Department of Transit. However, it was discovered that the daily usage was not collected and the parking space availability was dependent on new construction of parking lots, which would have to be manually collected to receive the numbers on available parking spaces over the years of 2017--2022. 

Understanding this issue, we determined that information on the semesterly sales of JMU parking permits would give us similar findings compared to the usage of the parking spaces, albeit not in the form of daily usage, and the parking permit data were thought to reflect private car usage on JMU's campus. There was a lack of data points for this data, though, since it was collected semesterly and the time period being studied was a 5-year time frame; thus, correlation of parking permit sales and public transit ridership was able to be calculated but it neither had a strong correlation present nor was it appropriate to generalize this analysis due to the low sample size. Furthermore, upon greater consideration it was realized that although students may drive their personal vehicles to JMU for classes if they do not live on-campus, these students would likely still utilize the inner-campus shuttle---which is a form of public transportation---during the day. We believe this invalidates the necessity of exploring the relationship between JMU parking permit sales and public transportation ridership a there is no clear way to separate those not riding public transportation on-campus but using a parking permit.

==> Sections/arcgis.tex <==
\subsection{ArcGIS}

ArcGIS is a website specializing in building maps by geographic census information. Using this platform, we created various layered maps that display public transportation routes as well as Harrisonburg SVI data.

\begin{figure}
    \includegraphics[width=0.75\textwidth]{Images/maps/arcgis_stops_svi.pdf}
    \captionof{figure}{A map of Harrisonburg displaying bus stops and SVI by census tract.}
    \label{fig:svi_map}
\end{figure}
